BURST: A Benchmark for Unifying Object Recognition, Segmentation and Tracking in Video

Multiple existing benchmarks involve tracking and segmenting objects in video e.g., Video Object Segmentation (VOS) and Multi-Object Tracking and Segmentation (MOTS), but there is little interaction between them due to the use of disparate benchmark datasets and metrics (e.g. J&F, mAP, sMOTSA). As a result, published works usually target a particular benchmark, and are not easily comparable to each another. We believe that the development of generalized methods that can tackle multiple tasks requires greater cohesion among these research sub-communities. In this paper, we aim to facilitate this by proposing BURST, a dataset which contains thousands of diverse videos with high-quality object masks, and an associated benchmark with six tasks involving object tracking and segmentation in video. All tasks are evaluated using the same data and comparable metrics, which enables researchers to consider them in unison, and hence, more effectively pool knowledge from different methods across different tasks. Additionally, we demonstrate several baselines for all tasks and show that approaches for one task can be applied to another with a quantifiable and explainable performance difference. Dataset annotations and evaluation code is available at: https://github.com/Ali2500/BURST-benchmark.

==> sections/checklist.tex <==
\clearpage

\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

==> tables/baselines_openworld.tex <==
\begin{table}
\centering{}
\setlength{\tabcolsep}{1.0pt}
\renewcommand{\arraystretch}{1.0}
\footnotesize

\caption{
Baseline results for the class-guided, open-world benchmark. Object detectors were trained on COCO.
%Detector Architectures: \textbf{MRCNN}: Mask-RCNN, \textbf{M2F}: Mask2Former.
}
% Preview source code for paragraph 0

\begin{tabular}{>{\centering}p{8em}>{\centering}p{5em}>{\centering}p{5em}>{\centering}p{5em}}
\toprule 
\multirow{2}{8em}{\raggedright{}\textbf{Method}} & \textbf{Common} & \textbf{Uncommon} & \textbf{All}\tabularnewline
\cmidrule{2-4} \cmidrule{3-4} \cmidrule{4-4} 
 & \centering{}$\mathrm{OWTA}$ & \centering{}$\mathrm{OWTA}$ & \centering{}$\mathrm{OWTA}$\tabularnewline
\midrule 
\raggedright{}Box Tracker & 66.9 & 25.7 & 60.3\tabularnewline
\raggedright{}STCN Tracker & 71.0 & 25.0 & 63.7\tabularnewline
\raggedright{}OWTB & 59.8 & 38.8 & 55.8\tabularnewline
\bottomrule
\end{tabular}

\label{tab:baselines_openworld}
\end{table}

==> tables/datasets_by_size.tex <==



\begin{table*}
\centering{}
\setlength{\tabcolsep}{1.3pt}
\renewcommand{\arraystretch}{1.0}
\scriptsize

\caption{\textbf{Datasets by Size.}
\label{tab:dataset_comparison_by_size}
}    
    
\begin{tabular}{cccccccccc}
\toprule 
 & \multicolumn{4}{c}{Training Size} &  & \multicolumn{4}{c}{Test/Val Size}\tabularnewline
\cmidrule{2-5} \cmidrule{3-5} \cmidrule{4-5} \cmidrule{5-5} \cmidrule{7-10} \cmidrule{8-10} \cmidrule{9-10} \cmidrule{10-10} 
 & Masks & Tracks & Frames & Vids &  & Masks & Tracks & Frames & Vids\tabularnewline
\midrule 
% {\color{gray}ImageNet-Vid} & {\color{gray}-} & {\color{gray}9,600} & {\color{gray}1,060,000} & {\color{gray}4,000} &  & {\color{gray}-} & {\color{gray}3154} & {\color{gray}438,210} & {\color{gray}1,314}\tabularnewline
% {\color{gray}UA-DETRAC} & {\color{gray}-} & {\color{gray}3,456} & {\color{gray}16,800} & {\color{gray}60} &  & {\color{gray}-} & {\color{gray}2,304} & {\color{gray}645,120} & {\color{gray}40}\tabularnewline
%{\color{gray}Waymo} & {\color{gray}-} & {\color{gray}176,046} & {\color{gray}159,600} & {\color{gray}798} &  & {\color{gray}-} & {\color{gray}77,654} & {\color{gray}70,400} & {\color{gray}352}\tabularnewline
% {\color{gray}TAO} & {\color{gray}-} & {\color{gray}2,950} & {\color{gray}18,400} & {\color{gray}500} &  & {\color{gray}-} & {\color{gray}14,202} & {\color{gray}88,578} & {\color{gray}2,407}\tabularnewline
%\midrule 
%{\color{gray}CityScapesVideo} & {\color{gray}196,100} & {\color{gray}39,220} & {\color{gray}13,530} & {\color{gray}2,706} &  & {\color{gray}57,715} & {\color{gray}11,543} & {\color{gray}3,975} & {\color{gray}795}\tabularnewline
%\midrule 
VOT & 0 & 0 & 0 & 0 &  & 19,903 & 62 & 19,903 & 62\tabularnewline
DAVIS & 13,246 & 179 & 4,440 & 60 &  & 19,906 & 269 & 6,660 & 90\tabularnewline
YT-VOS & 174,393 & 6,459 & 93,717 & 3,471 &  & 48,843 & 1,809 & 26,514 & 982\tabularnewline
BDD & 110,571 & 5,400 & 12,000 & 60 &  & 55,286 & 2,700 & 6,000 & 30\tabularnewline
KITTI & 26,904 & 530 & 5,027 & 12 &  & 63,394 & 637 & 8,672 & 30\tabularnewline
MOTS-Challenge & 26,894 & 228 & 2,862 & 4 &  & 32,269 & 328 & 3044 & 4\tabularnewline
YT-VIS & 102,119 & 3,791 & 60,426 & 2,238 &  & 29,431 & 1,092 & 17,415 & 645\tabularnewline
UVO & 479,236 & \textbf{66,366} & 38,994 & \textbf{5400} &  & 486,868 & \textbf{65,702} & 39,615 & \textbf{5,346}\tabularnewline
TSUnami (Ours) & \textbf{3,256,800} & 2,950 & \textbf{552,000} & 500 &  & \textbf{522,634} & 14,202 & \textbf{88,578} & 2,407\tabularnewline
\bottomrule
\end{tabular}


\end{table*}


==> tables/expanded_baselines_openworld_test.tex <==
\begin{table*}[h]
\vspace{10pt}
\caption{Extended baseline results for the open-world class-guided task for the test set.}
\label{tab:extended_openworld_baselines_test}
\centering
\footnotesize
\vspace{4pt}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{0.8\linewidth}{lp{3pt}YYYp{3pt}YYYp{3pt}YYY}
\toprule
\multirow{2}{*}{Baseline Method} & & \multicolumn{3}{c}{All} & & \multicolumn{3}{c}{Common} & & \multicolumn{3}{c}{Uncommon} \\
\cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
                & & $\mathrm{DetRe}$ & $\mathrm{AssA}$ & $\mathrm{OWTA}$ & & $\mathrm{DetRe}$ & $\mathrm{AssA}$ & $\mathrm{OWTA}$ & & $\mathrm{DetRe}$ & $\mathrm{AssA}$ & $\mathrm{OWTA}$ \\
\cmidrule{1-1} \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
STCN Tracker           & & 61.6 & 54.1  & 57.5  & & 71.5  & 55.7  & 62.9 & & 21.0  & 28.6  & 23.9  \\
Box Tracker            & & 61.5 & 51.1  & 55.9  & & 71.4  & 52.5  & 61.0 & &        &       &       \\
OWTB~\cite{liu22OWTB}  & &      &       &       & &       &       &      & &       &       &       \\
\bottomrule
\end{tabularx}

\end{table*}

==> tables/expanded_baselines_openworld_validation.tex <==
\begin{table*}[h]
\vspace{10pt}
\caption{Extended baseline results for the open-world class-guided task for the validation set.}
\label{tab:extended_openworld_baselines_validation}
\centering
\footnotesize
\vspace{4pt}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{0.8\linewidth}{lp{3pt}YYYp{3pt}YYYp{3pt}YYY}
\toprule
\multirow{2}{*}{Baseline Method} & & \multicolumn{3}{c}{All} & & \multicolumn{3}{c}{Common} & & \multicolumn{3}{c}{Uncommon} \\
\cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
                & & $\mathrm{DetRe}$ & $\mathrm{AssA}$ & $\mathrm{OWTA}$ & & $\mathrm{DetRe}$ & $\mathrm{AssA}$ & $\mathrm{OWTA}$ & & $\mathrm{DetRe}$ & $\mathrm{AssA}$ & $\mathrm{OWTA}$ \\
\cmidrule{1-1} \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
%
STCN Tracker           & & 67.0 & 62.6  & 64.6  & & 78.8 & 64.1  & 71.0  & & 20.0  & 33.3  & 25.0  \\
Box Tracker            & & 66.9 & 55.8  & 60.9  & & 78.7 & 57.1  & 60.9  & & 20.1  & 30.5  & 24.0  \\
OWTB~\cite{liu22OWTB}  & &      &       &       & &       &       &      & &       &       &       \\
%
\bottomrule
\end{tabularx}

\end{table*}

==> tables/expanded_baselines_test.tex <==
\begin{table*}[h]
\vspace{10pt}
\centering{}
\setlength{\tabcolsep}{4.0pt}
% \renewcommand{\arraystretch}{1.0}
\newcommand\RotText[1]{\rotatebox{90}{\parbox{2cm}{\centering#1}}}
\footnotesize
%\scriptsize
% \small
\def\metricFontSize{\tiny}
\def\streamFontSize{\scriptsize}

\caption{
Extended baseline results for the test set with multiple metrics.
Evaluation metrics are reported separately for `common', `uncommon' and `all' classes. 
Object detector training data: \textbf{*}: COCO, \textbf{$\dagger$}: LVIS. 
}
\vspace{4pt}

% Preview source code for paragraph 0
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{\textwidth}{cclYYYcYp{5pt}YYYcYp{5pt}YYYcY}
% Preview source code for paragraph 0
\toprule 
%
 & & \multirow{2}{*}{Baseline Method} & \multicolumn{5}{c}{All} &  & \multicolumn{5}{c}{Common} &  & \multicolumn{5}{c}{Uncommon}\\
\cmidrule{4-8} \cmidrule{10-14} \cmidrule{16-20}
 &  &  & \metricFontSize{}$\mathrm{DetA}$ & \metricFontSize{}$\mathrm{AssA}$ & \metricFontSize{}$\mathrm{HOTA}$ & \metricFontSize{}$\mathrm{HOTA}^\text{obj}$ & \metricFontSize{} mAP &  & \metricFontSize{}$\mathrm{DetA}$ & \metricFontSize{}$\mathrm{AssA}$ & \metricFontSize{}$\mathrm{HOTA}$ & \metricFontSize{}$\mathrm{HOTA}^\text{obj}$ & \metricFontSize{} mAP &  & \metricFontSize{}$\mathrm{DetA}$ & \metricFontSize{}$\mathrm{AssA}$ & \metricFontSize{}$\mathrm{HOTA}$ & \metricFontSize{}$\mathrm{HOTA}^\text{obj}$ & \metricFontSize{} \metricFontSize{} mAP\\
%
\cmidrule{1-8} \cmidrule{10-14} \cmidrule{16-20} 
\multirow{7}{10pt}{\centering{}\rotatebox{90}{\parbox{2cm}{\streamFontSize{}  \centering Exemplar-guided}}} & \multirow{2}{*}{\centering{}Mask} & %
%
STCN~\cite{Cheng21stcn} & 48.8 & 57.3 & 52.4 & 60.7 & 34.4 &  & 45.0 & 59.2 & 51.1 & 61.0 & 30.0 &  & 49.6 & 57.0 & 52.7 & 59.5 & 35.3\\
 &  & Box Tracker{*}~\cite{luiten2020trackeval} & 12.1 & 17.2 & 14.1 & 44.4 & 3.5 &  & 21.9 & 37.3 & 28.0 & 48.5 & 9.2 &  & 10.2 & 13.2 & 11.4 & 16.9 & 2.4\\
\cmidrule{2-8} \cmidrule{10-14} \cmidrule{16-20} 
 & \multirow{3}{*}{\centering{}Box} & STCN (Pointrend~\cite{Kirillov20pointrend}) & 41.9 & 51.7 & 46.0 & 58.1 & 25.6 &  & 42.2 & 58.0 & 48.9 & 59.0 & 26.2 &  & 41.9 & 50.5 & 45.4 & 53.6 & 25.4\\
 &  & STCN (Matched Det{*}) & 20.6 & 32.9 & 25.0 & 53.9 & 13.6 &  & 33.1 & 55.5 & 41.9 & 56.6 & 20.5 &  & 18.1 & 28.4 & 21.7 & 36.6 & 12.2\\
 &  & Box Tracker{*} & 11.6 & 16.9 & 13.6 & 44.2 & 3.0 &  & 21.5 & 37.2 & 27.7 & 48.3 & 8.3 &  & 9.6 & 12.8 & 10.8 & 17.0 & 1.9\\
\cmidrule{2-8} \cmidrule{10-14} \cmidrule{16-20}
 & \multirow{2}{*}{\centering{}Point} & STCN (Matched Det{*}) & 20.6 & 32.5 & 24.9 & 49.6 & 12.5 &  & 30.8 & 53.8 & 39.5 & 52.3 & 17.7 &  & 18.6 & 28.3 & 22.0 & 34.6 & 11.5\\
 &  & Box Tracker{*} & 8.0 & 14.1 & 10.1 & 41.6 & 2.5 &  & 17.8 & 36.1 & 24.4 & 45.5 & 6.7 &  & 6.1 & 9.7 & 7.3 & 16.1 & 1.7\\
\midrule 
\multirow{4}{10pt}{\centering{}\rotatebox{90}{\parbox{1.5cm}{\streamFontSize{} \centering Class-guided}}} & \multirow{2}{*}{\centering{}Common} & STCN Tracker{*} & - & - & - & - & - &  & 37.1 & 34.9 & 34.6 & 58.8 & 6.8 &  & - & - & - & - & -\\
 &  & Box Tracker{*} & - & - & - & - & - &  & 37.1 & 35.5 & 34.3 & 56.9 & 6.8 &  & - & - & - & - & -\\
\cmidrule{2-8} \cmidrule{10-14} \cmidrule{16-20}
 & \multirow{2}{*}{\centering{}Long-Tail} & STCN Tracker$^{\dagger}$ & 5.4 & 4.6 & 4.5 & 13.4 & 0.3 &  & 19.6 & 16.7 & 17.1 & 14.3 & 1.7 &  & 2.6 & 2.2 & 2.0 & 8.0 & 0.0\\
 &  & Box Tracker$^{\dagger}$ & 5.4 & 6.8 & 5.7 & 15.4 & 0.3 &  & 19.6 & 23.2 & 20.1 & 16.3 & 1.7 &  & 2.6 & 3.6 & 2.9 & 10.7 & 0.0\\
\bottomrule
\end{tabularx}


\label{tab:expanded_baselines_test}
\end{table*}

==> tables/expanded_baselines_validation.tex <==
\begin{table*}[h]
\centering{}
\setlength{\tabcolsep}{4.0pt}
% \renewcommand{\arraystretch}{1.0}
\newcommand\RotText[1]{\rotatebox{90}{\parbox{2cm}{\centering#1}}}
\footnotesize
%\scriptsize
% \small
\def\metricFontSize{\tiny}
\def\streamFontSize{\scriptsize}

\caption{
Extended baseline results for the validation set with multiple metrics.
Evaluation metrics are reported separately for `common', `uncommon' and `all' classes. 
Object detector training data: \textbf{*}: COCO, \textbf{$\dagger$}: LVIS. 
}
\vspace{4pt}

% Preview source code for paragraph 0
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{\textwidth}{cclYYYcYp{5pt}YYYcYp{5pt}YYYcY}
%{>{\raggedright}p{3em}>{\raggedright}p{7em}>{\raggedright}m{10em}>{\centering}p{3em}>{\centering}p{3em}>{\centering}p{3em}>{\centering}p{4em}>{\centering}p{5em}>{\centering}p{1pt}>{\centering}p{3em}>{\centering}p{3em}>{\centering}p{3em}>{\centering}p{4em}>{\centering}p{3em}>{\centering}p{1pt}>{\centering}p{3em}>{\centering}p{3em}>{\centering}p{3em}>{\centering}p{4em}>{\centering}p{3em}}
\toprule 
%
 & & \multirow{2}{*}{Baseline Method} & \multicolumn{5}{c}{All} &  & \multicolumn{5}{c}{Common} &  & \multicolumn{5}{c}{Uncommon}\\
\cmidrule{4-8} \cmidrule{10-14} \cmidrule{16-20}
 &  &  & \metricFontSize{}$\mathrm{DetA}$ & \metricFontSize{}$\mathrm{AssA}$ & \metricFontSize{}$\mathrm{HOTA}$ & \metricFontSize{}$\mathrm{HOTA}^\text{obj}$ & \metricFontSize{} $\mathrm{mAP}$ &  & \metricFontSize{}$\mathrm{DetA}$ & \metricFontSize{}$\mathrm{AssA}$ & \metricFontSize{}$\mathrm{HOTA}$ & \metricFontSize{}$\mathrm{HOTA}^\text{obj}$ & \metricFontSize{} $\mathrm{mAP}$ &  & \metricFontSize{}$\mathrm{DetA}$ & \metricFontSize{}$\mathrm{AssA}$ & \metricFontSize{}$\mathrm{HOTA}$ & \metricFontSize{}$\mathrm{HOTA}^\text{obj}$ & \metricFontSize{} \metricFontSize{} $\mathrm{mAP}$\\
\cmidrule{1-8} \cmidrule{10-14} \cmidrule{16-20} 
\multirow{7}{10pt}{\centering{}\rotatebox{90}{\parbox{2cm}{\streamFontSize{}  \centering Exemplar-guided}}} & \multirow{2}{*}{\centering{}Mask} & %
STCN~\cite{Cheng21stcn}                    &  46.1    &   54.9    &   49.8    &   59.2    &   33.3    &   &   44.7    &   62.5    &   52.2    &   60.1    &   27.5    &   &   46.4    &   53.1    &   49.2    &   54.8    &   34.8\\
 &  & %
 Box Tracker{*}~\cite{luiten2020trackeval}         &  15.1    &   22.5    &   18.0    &   47.7    &   12.5    &   &   28.7   &    46.3    &   35.8    &   52.3    &   12.5    &   &   11.8    &   16.6    &   13.6   &    18.8    &   4.4\\
\cmidrule{2-8} \cmidrule{10-14} \cmidrule{16-20} 
 & \multirow{3}{*}{\centering{}Box} & %
STCN (PointRend~\cite{Kirillov20pointrend})        &  41.1    &   51.1    &   45.8    &   57.1    &   26.7    &   &   40.9    &   60.2    &   48.9    &   58.5    &   23.5    &   &   41.1    &   48.8    &   44.3    &   50.9    &   27.5\\
 &  & %
STCN (Matched Det{*})   &  20.0    &   32.4    &   24.5    &   54.4    &   13.3    &    &   38.7    &   60.8    &   47.6    &   57.6    &   22.7    &   &   15.4    &   25.3    &   18.7    &   34.2    &   11.0\\
 &  & Box Tracker{*} & 10.9 & 18.8 & 13.7 & 48.6 & 4.4 &  & 27.1 & 45.0 & 34.2 & 52.8 & 10.8 &  & 6.9 & 12.2 & 8.6 & 18.3 & 2.8\\
\cmidrule{2-8} \cmidrule{10-14} \cmidrule{16-20}
 & \multirow{2}{*}{\centering{}Point} & STCN (Matched Det{*}) & 19.9 & 32.1 & 24.4 & 48.4 & 12.8 &  & 34.4 & 59.0 & 44.0 & 51.6 & 20.6 &  & 16.3 & 25.4 & 19.4 & 31.4 & 10.8\\
 &  & Box Tracker{*} & 9.9 & 17.6 & 12.7 & 43.7 & 3.2 &  & 24.2 & 43.7 & 31.7 & 48.0 & 9.7 &  & 6.3 & 11.2 & 7.9 & 17.1 & 1.6\\
\cmidrule{1-8} \cmidrule{10-14} \cmidrule{16-20} 
\multirow{4}{10pt}{\centering{}\rotatebox{90}{\parbox{1.5cm}{\streamFontSize{} \centering Class-guided}}} & \multirow{2}{*}{\centering{}Common} & STCN Tracker{*} & - & - & - & - & - &  & 51.7 & 51.9 & 51.2 & 66.8 & 13.6 &  & - & - & - & - & -\\
 &  & Box Tracker{*} &  &  &  &  &  &  & 51.7 & 43.0 & 45.5 & 62.9 & 9.9 &  & - & - & - & - & -\\
\cmidrule{2-8} \cmidrule{10-14} \cmidrule{16-20}
 & \multirow{2}{*}{\centering{}Long-Tail} & STCN Tracker$^{\dagger}$ & 8.0 & 13.4 & 5.5 & 13.5 & 0.9 &  & 27.0 & 13.4 & 17.5 & 14.4 & 0.7 &  & 3.2 & 2.4 & 2.5 & 8.9 & 0.6\\
 &  & Box Tracker$^{\dagger}$ & 8.3 & 29.5 & 8.2 & 18.6 & 1.4 &  & 28.0 & 29.5 & 27.0 & 19.8 & 3.0 &  & 3.4 & 4.3 & 3.6 & 11.7 & 0.9\\
\bottomrule
\end{tabularx}









\label{tab:expanded_baselines_validation}
\end{table*}

==> tables/training_annotations_stats.tex <==
\begin{table}[h]
    \centering
    \scriptsize
    
    \caption{Statistics for training set annotation/densification. \todo{How to present this exactly?}}
    \vspace{5pt}

    \begin{tabular}{lc}
\toprule 
Setting & \#Masks\tabularnewline
\midrule
GT at 1fps & 60095\tabularnewline
Manual annotations for 1fps $\rightarrow$ 3fps & 20582\tabularnewline
Bad-auto annotations for 1fps $\rightarrow$ 3fps & 20582\tabularnewline
Good auto-annotations for 1fps $\rightarrow$ 3fps & 98347\tabularnewline
Total auto-annotations for 3fps $\rightarrow$ 6fps & 177906\tabularnewline
Bad auto-annotations for 3fps $\rightarrow$ 6fps & 27601\tabularnewline
Bad auto-annotations for 1fps $\rightarrow$ 6fps & 54630\tabularnewline
Bad auto-annotations for 1fps $\rightarrow$ 3fps $\rightarrow$ 6fps & 20582 + 27601 = 48183\tabularnewline
\bottomrule
\end{tabular}
    
    \label{tab:training_annotations_stats}
\end{table}
